Predicting long time contributors with knowledge units of programming languages: an empirical study

Predicting potential long-time contributors (LTCs) early allows project maintainers to effectively allocate resources and mentoring to enhance their development and retention. Mapping programming language expertise to developers and characterizing projects in terms of how they use programming languages can help identify developers who are more likely to become LTCs. However, prior studies on predicting LTCs do not consider programming language skills. This paper reports an empirical study on the usage of knowledge units (KUs) of the Java programming language to predict LTCs. A KU is a cohesive set of key capabilities that are offered by one or more building blocks of a given programming language. We build a prediction model called KULTC, which leverages KU-based features along five different dimensions. We detect and analyze KUs from the studied 75 Java projects (353K commits and 168K pull requests) as well as 4,219 other Java projects in which the studied developers previously worked (1.7M commits). We compare the performance of KULTC with the state-of-the-art model, which we call BAOLTC. Even though KULTC focuses exclusively on the programming language perspective, KULTC achieves a median AUC of at least 0.75 and significantly outperforms BAOLTC. Combining the features of KULTC with the features of BAOLTC results in an enhanced model (KULTC+BAOLTC) that significantly outperforms BAOLTC with a normalized AUC improvement of 16.5%. Our feature importance analysis with SHAP reveals that developer expertise in the studied project is the most influential feature dimension for predicting LTCs. Finally, we develop a cost-effective model (KULTC_DEV_EXP+BAOLTC) that significantly outperforms BAOLTC. These encouraging results can be helpful to researchers who wish to further study the developers' engagement/retention to FLOSS projects or build models for predicting LTCs.

==> emse-template/setup.tex <==
% ------------- Packages Used --------------------------------------------------
% They help us to produce a better looking document ;-)
% ------------------------------------------------------------------------------

% Comment the following line before compiling the final version
%\synctex
\RequirePackage{fix-cm}

\usepackage{caption}
\usepackage{multirow}
\usepackage{balance}
\usepackage{graphicx}
\usepackage{alltt}
\usepackage{relsize}
%\usepackage{xspace}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{paralist}
\usepackage{pbox}
%\usepackage{cleveref}
\usepackage[most]{tcolorbox}
\newcommand{\tabitem}{~~\llap{\textbullet}~~}

\usepackage{array}
\usepackage{amsmath}
\usepackage{multirow}
%\usepackage{array}
\usepackage{verbatim}
%\usepackage[table]{xcolor}
\usepackage{rotating}
%\usepackage{subcaption}
%\usepackage{subfigure}
\usepackage[tight,footnotesize]{subfigure}

%\usepackage{capt-of}
%\usepackage{pifont}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage[latin1]{inputenc}
%\usepackage{times}
%\usepackage{colortbl}
\usepackage{boxedminipage}
\usepackage{float}
\usepackage{cite}
\usepackage{fancyvrb}



\usepackage{balance}

\usepackage{fancybox}%for \hypobox
\usepackage{listings}
\usepackage{array}
\usepackage{afterpage}
\usepackage{pdflscape}
\usepackage{lscape}
\usepackage{rotating}

\usepackage[T1,hyphens]{url}
%\usepackage[colorlinks,urlcolor=blue]{hyperref}


%\hypersetup{
%	colorlinks=true,
%	linkcolor=blue,
%	filecolor=blue,      
%	urlcolor=blue,
%	citecolor=blue,
%}
%\urlstyle{same}

\usepackage{textcomp}
%\usepackage{latexsym}
%\usepackage{amssymb}
%\usepackage{stmaryrd}
%\usepackage{euscript}
%\usepackage{wasysym}
%\usepackage{pifont}
%\usepackage{manfnt}
%\usepackage{undertilde}
%\usepackage{ifsym}
%\usepackage{tipa}
%\usepackage{txfonts}
%\usepackage{skak}
%\usepackage{skull}
%\usepackage{eurosym}
%\usepackage{yfonts}
%\usepackage{mathdots}
%\usepackage{trsym}
%\usepackage{upgreek}
%\usepackage{chemarr}
%\usepackage{accents}
%\usepackage{nicefrac}
%\usepackage{bm}


%\usepackage{pdfsync}

%   ACM Style
%\usepackage{lcsect}
% ------------------------------------------------------------------------------






% ------------ Color Definitions -----------------------------------------------
% Whatever colors we need
% ------------------------------------------------------------------------------
\definecolor{mygray}{rgb}{0.7,0.7,0.7}
% ------------------------------------------------------------------------------






% ---------- Special commands for annotating the paper's text ------------------
\let\mymarginpar\marginparm
\marginparwidth=1cm
\marginparsep=5pt
\newcommand{\todo}[1]{\textcolor{red}{\textbf{[[#1]]}}}
\def\TODO#1{\noindent\colorbox{yellow}{\bf \textcolor{red}{TODO: #1}}}
\newcommand{\hint}[1]{\textcolor{blue}{\textbf{#1}}}
\def\fig#1{Figure~\ref{#1}}
\def\tab#1{Table~\ref{#1}}
\def\eqn#1{Equation~\ref{#1}}
\def\sec#1{Section~\ref{#1}}

\pagenumbering{arabic}
\newcommand{\reviewer}[1]{\textcolor{DeepPink1}{{\it [Reviewer says: #1]}}}
\newcommand{\safwat}[1]{\textcolor{red}{{\it [Safwat says: #1]}}}
\newcommand{\ian}[1]{\textcolor{blue}{{\it [Ian says: #1]}}}
\newcommand{\nic}[1]{\textcolor{WildStrawberry}{{\it [Nico says: #1]}}}
\newcommand{\ahmed}[1]{\textcolor{orange}{{\it [Ahmed says: #1]}}}
\newcommand{\ahsan}[1]{\textcolor{blue}{{\it \textbf{[Ahsan says: #1]}}}}
\newcommand{\fix}[1]{\textcolor{blue}{{\it \textbf{[Fix: #1]}}}}
\newcommand{\cp}[1]{\textcolor{red}{{\it [Cor-Paul says: #1]}}}
\newcommand{\kla}[1]{\textcolor{red}{{\it [Kla says: #1]}}}

\newcommand{\myfoot}[1]{\footnote{\scriptsize #1}}
\newcommand{\myurl}[1]{\myfoot{\url{#1}}}
\newcommand{\Ra}{{$\Rightarrow$}}
\newcommand{\ra}{{$\rightarrow$}}
\newcommand{\La}{{$\Leftarrow$}}
\newcommand{\la}{{$\leftarrow$}}
\newcommand{\lra}{{$\leftrightarrow$}}
\newcommand{\LRa}{{$\Leftrightarrow$}}
%\newcommand{\todo}{\bram{todo}}

\newenvironment{myindentpar}[1]%
{\begin{list}{}%
         {\setlength{\leftmargin}{#1}}%
         \item[]%
}
{\end{list}}

% \AtBeginDocument{%
%    \renewcommand{\figurename}{Figure}%
%    \newcommand{\subfigureautorefname}{\figureautorefname}%for using subfig
% %   \renewcommand{\tablename}{TABLE}%
%    \renewcommand{\tablename}{Table}%
%    \renewcommand{\subsectionautorefname}{Section}%
%    \renewcommand{\sectionautorefname}{Section}%
% }

% Hypothesis box	
% ------------------------------------------------------------------------------	
\newcommand{\hypobox}[1]{\begin{center}%	
	\noindent\thicklines\setlength{\fboxsep}{7pt}%	
	\cornersize{0}\Ovalbox{\begin{minipage}{3.1in}%	
	\vspace{-0.1cm}
	\textit{#1}
	\vspace{-0.1cm}
	\end{minipage}} \end{center}}	
% ------------------------------------------------------------------------------




% ------------------------- SYMBOLS OF SELF NAMES OFTEN USED -------------------
\newcommand{\APACHE}{{\small APACHE}\xspace}
\newcommand{\BUGZILLA}{{\small BUGZILLA}\xspace}
\newcommand{\ECLIPSE}{{\small ECLIPSE}\xspace}
\newcommand{\ASPECTJ}{{\small ASPECTJ}\xspace}
\newcommand{\JDT}{{\small JDT}\xspace}
\newcommand{\GNU}{{\small GNU}\xspace}
\newcommand{\MOZILLA}{{\small MOZILLA}\xspace}
\newcommand{\THUNDERBIRD}{{\small THUNDERBIRD}\xspace}
\newcommand{\JAVA}{{\small Java}\xspace}
\newcommand{\GNOME}{{\small GNOME}\xspace}
\newcommand{\PG}{{\small PostgreSQL}\xspace}
\newcommand{\SIM}{{\small SimScan}\xspace}


\newcommand{\NEGDIFF}{{\emph{Neg}$_{\text{\emph{Diff}}}$}}



% Anything else, e.g., \NAME{MICROSOFT}
\newcommand{\NAME}[1]{{\small #1}\xspace}
% ------------------------------------------------------------------------------




% ----------------------- Computer Science lol ---------------------------------
% Variable, function, and program names
% ------------------------------------------------------------------------------
\newcommand{\smalltt}[1]{\ifmmode{\mbox{\smaller\texttt{#1}}}\else{\smaller\tt #1}\fi}
\newcommand{\code}[1]{\smalltt{#1}}
\newcommand{\var}[1]{\code{#1}}
\newcommand{\func}[1]{\code{#1}}
\newcommand{\proc}[1]{\code{#1}}
\newcommand{\prog}[1]{\code{#1}}
\newcommand{\type}[1]{\code{#1}}
\newcommand{\progpt}[1]{\code{#1}}

\newcommand{\mypar}[1]{\vspace{.1cm}\noindent \textbf{#1}}
\newcommand{\myxpar}[1]{\vspace{.1cm}\noindent \textbf{#1}\newline}
% ------------------------------------------------------------------------------





% ----------- Things to remember -----------------------------------------------
\newenvironment{mynote}%
{ \medskip
  \noindent
  \let\emph=\textbf
  \begin{boxedminipage}{\columnwidth}\em}%
{ \end{boxedminipage}}
% ------------------------------------------------------------------------------






% -------------------- Use bars ------------------------------------------------
% These macros are for advanced presentation of results by shaded bars only!
% © Tom Zimmermann, 2008
% ------------------------------------------------------------------------------
\newdimen\qdx
\newdimen\qda
\newdimen\qdb
\def\rrrr#1#2#3#4{\newdimen\qd\qd=#4 % length of bar for 1.0
\qdx=\qd\multiply\qdx by 5\divide\qdx by 4
\qda=\qd
\qdb=\qd
\multiply\qda by #1\divide\qda by #3\multiply\qdb by #2\divide\qdb by #3\advance\qdb by -\qda
    \leavevmode\hbox to \qdx{\hfil\vbox{%
    \hbox{\vrule\vbox{\hrule\hbox to 1\qd
            {\vrule depth0pt height0.7ex width \qda\color{mygray}%
 \vrule depth0pt height0.7ex width \qdb\hfill}\hrule}\vrule}
    }\hfil}}
\def\rrr#1#2#3{\rrrr{#1}{#2}{#3}{0.8cm}}
% -------------------------------------------------------------------------






% ------------ Graphics Hacks --------------------------------------------------
% Use these settings if Figures tend to get their one separate pages
% ------------------------------------------------------------------------------
% \renewcommand{\topfraction}{0.85}
% \renewcommand{\textfraction}{0.1}
% \renewcommand{\floatpagefraction}{0.75}
% ------------------------------------------------------------------------------





% ------------------ Biblio Hack -----------------------------------------------
% Use these settings if the References take too much space
% ------------------------------------------------------------------------------
\let\oldthebibliography=\thebibliography
  \let\endoldthebibliography=\endthebibliography
  \renewenvironment{thebibliography}[1]{%
%	\vspace{-0.3cm}
    \begin{oldthebibliography}{#1}%
%	\vspace{-0.2cm}
       \setlength{\parskip}{0ex}%
       \setlength{\itemsep}{0ex}%
%	\bibfont
  }%
  {%
    \end{oldthebibliography}%
  }
% ------------------------------------------------------------------------------





% -------------- Floats Redefined ----------------------------------------------
% Use these settings to change the whitespace between floats and text
% ------------------------------------------------------------------------------

% \setlength\dblfloatsep{1pt}
% \setlength\floatsep{1pt}
% \setlength\textfloatsep{5pt}
% \setlength\dbltextfloatsep{5pt}

% \renewcommand\floatpagefraction{.9}
% \renewcommand\topfraction{.9}
% \renewcommand\bottomfraction{.9}
% \renewcommand\textfraction{.1}
% \setcounter{totalnumber}{50}
% \setcounter{topnumber}{50}
% \setcounter{bottomnumber}{50}
% ------------------------------------------------------------------------------



% The custom defined cell types, I needed this to make the headers centered but the remaining of the column is right or left justified.
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\usepackage{tikz}
\usetikzlibrary{shapes.geometric,calc}

\newcommand\score[2]{
	\pgfmathsetmacro\pgfxa{#1+1}
	\tikzstyle{scorestars}=[star, star points=5, star point ratio=2.25, draw,inner sep=0.15em,anchor=outer point 3]
	\begin{tikzpicture}[baseline]
	\foreach \i in {1,...,#2} {
		\pgfmathparse{(\i<=#1?"yellow":"gray")}
		\edef\starcolor{\pgfmathresult}
		\draw (\i*1em,0) node[name=star\i,scorestars,fill=\starcolor]  {};
	}
	\pgfmathparse{(#1>int(#1)?int(#1+1):0}
	\let\partstar=\pgfmathresult
	\ifnum\partstar>0
	\pgfmathsetmacro\starpart{#1-(int(#1))}
	\path [clip] ($(star\partstar.outer point 3)!(star\partstar.outer point 2)!(star\partstar.outer point 4)$) rectangle 
	($(star\partstar.outer point 2 |- star\partstar.outer point 1)!\starpart!(star\partstar.outer point 1 -| star\partstar.outer point 5)$);
	\fill (\partstar*1em,0) node[scorestars,fill=yellow]  {};
	\fi
	
	,\end{tikzpicture}
}

\newcommand{\smallnum}[1]{$^{\tiny {\textbf #1}}$}

\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newcommand{\specialcellLeft}[2][t]{%
	\begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}

\usepackage{threeparttable, tablefootnote}

\newtcolorbox[auto counter]{summary_RQ1}[1][]{title={\bfseries Summary of RQ1},enhanced,
	coltitle=black,
	top=0.17in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=lightgray},#1}

\newtcolorbox[auto counter]{summary_RQ2}[1][]{title={\bfseries Summary of RQ2},enhanced,
	coltitle=black,
	top=0.17in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=lightgray},#1}
	
\newtcolorbox[auto counter]{summary_RQ3}[1][]{title={\bfseries Summary of RQ3},enhanced,
	coltitle=black,
	top=0.17in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=lightgray},#1}

==> sections/Bios.tex <==
\vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/Bios/ahsan.jpg}}]
    {\scriptsize Md Ahasanuzzaman}\scriptsize is currently a Ph.D. student in the Software Analysis and Intelligence Lab (SAIL) at Queen's University, Canada. His research interests include mining software repositories, source code analysis (e.g., mobile apps, Java applications), natural language processing and machine learning. His studies got published in top Software Engineering venues (e.g., TSE, EMSE,  MSR and SANER). He obtained his BSc from the University of Dhaka in Bangladesh. He has been awarded prestigious awards, such as Deans scholarship award and Prime Minister Gold Medal for his outstanding achievements in the B.Sc program. More information at: \url{https://scholar.google.ca/citations?hl=en&pli=1&user=7H2HIWgAA}
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/Bios/gus-bw.png}}]
	{\scriptsize Gustavo A. Oliva} \scriptsize is an Adjunct Professor at the School of Computing of Queen's University in Canada. Gustavo leads the blockchain research team at the Software Analysis and Intelligence Lab (SAIL). In addition to blockchain, he also conducts empirical studies in the fields of software ecosystems (e.g., npm), software evolution, and explainable AI. Gustavo received his MSc and PhD degrees from the University of São Paulo (USP) in Brazil under the supervision of professor Dr. Marco Aur{é}lio Gerosa. More information at: \url{https://www.gaoliva.com}
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/Bios/ahmed.jpg}}]
    {\scriptsize Ahmed E. Hassan} \scriptsize is a fellow of ACM, IEEE, AAIA, and NSERC Steacie. Hassan is a laureate of the Mustafa Prize, recognized as equivalent in prestige as a Nobel by Science Magazine. Hassan is an IEEE TCSE Distinguished Educator and an ACM SIGSOFT Influential Educator. He is a member of Canada’s Royal Society (New College) and a Canada Research Chair (CRC) in Software Analytics at the School of Computing at Queen’s University Canada. He is ranked in the top 0.03\% highest impact scientist across all disciplines and years of SCOPUS data. He is the world’s most prolific SE researcher in the past decade. 30+ of his prior trainees are professors in top research-intensive universities in every continent. More information at: \url{http://sail.cs.queensu.ca}
\end{IEEEbiography}

==> sections/Findings.tex <==
\section{Findings}
\label{sec:Findings}

%We linked the RQs' findings here

\input{sections/Findings-RQ1}
\input{sections/Findings-RQ2}
\input{sections/Findings-RQ3}

==> sections/Preliminary_Study.tex <==
\section{Preliminary Study: \PrelimStudy}
\label{sec:Preliminary_Study}

\noindent \textbf{Motivation.} Motivation of preliminary study.

\smallskip \noindent \textbf{Approach.} Approach of our preliminary Study

\smallskip \noindent \textbf{Findings.} \observation{Key observation 1} Details of the observation 1.



\smallskip \observation{Key observation 2} Details of the observation 2.
\begin{footnotesize}
	\begin{mybox}{Summary}
		\textbf{\PrelimStudy}
		\tcblower
		Summary results of our preliminary study.
	\end{mybox}
\end{footnotesize}

==> sections/temp.tex <==
\begin{itemize}[itemsep=3pt, wide = 0pt, topsep=1pt, listparindent=\parindent, label=$\bullet$]
    \item {\textit{Step 1) Filter the PR dataset.}}

    \item {\textit{Step 2) Construct KULTC model for classifying LTCs using KUs.}}
    
    To construct the KULTC model, we begin by selecting key features along five distinct dimensions. These dimensions are broadly classified into two primary categories: the Project dimension and the Expertise dimension. We briefly explain KU features of each dimension below:

    \noindent\textbf{Project Dimension.} This dimension refers to the KU profile of a project that we use to construct KULTC. We create KU profiles for two types of projects. Firstly, we create a KU profile for the current project of interest (i.e., a project from our studied project) where the newcomer submits his/her first commit. Secondly, we create a KU profile for historical projects in which the newcomer previously worked on. We detail our approach below:

    \textbf{(1) KU profile for the current project.} In this section, we briefly explain how we construct a KU profile for the current project where the developer submits his/her first commit. For each of our selected developers $D$, we first select the project $P$ (from the studied projects) in which the developer submits a commit. Next, we identify the first commit ($C_{i}$) of $D$ that the developer submits to $P$. Then, we select the  commit $C_{i-1}$ which is immediately preceding to $C_{i}$. Finally, we determine the occurrences of KUs on each Java files of the commit $C_{i-1}$ and construct a 28-position KU vector that represents the KU profile of the current project $P$ for developer $D$. 

    \textbf{(2) KU profile for historical projects.} For each of the selected developer $D$, we first select the project $P$ (from the studied projects) in which the developer $D$ submits a commit. Then, we identify the first commit ($C_{i}$) of $D$ that the developer submits to $P$. Next, we collect all the projects in which the developer $D$ contributed to by sending a GET request to the following URL using GitHub APIs:~\texttt{https://api.github.com/users/github-user-name/repos?per\_page=100}. 
    
    



    \noindent\textbf{Expertise Dimension.}



    \item {\textit{Step 3) Construct baseline models for classifying LTCs.}}
    \item {\textit{Step 4) Evaluate a model's performance.}}
        \begin{itemize}[itemsep=3pt, wide = 0pt, topsep=0pt, listparindent=\parindent]
            \item \textit{Step 4.1) Generate bootstrap samples. }
        \end{itemize}
    \item {\textit{Step 5) Compare model's performance.}}
\end{itemize}

